Truthful Online Scheduling of Cloud Workloads under Uncertainty

Cloud computing customers often submit repeating jobs and computation pipelines on \emph{approximately} regular schedules, with arrival and running times that exhibit variance. This pattern, typical of training tasks in machine learning, allows customers to partially predict future job requirements. We develop a model of cloud computing platforms that receive statements of work (SoWs) in an online fashion. The SoWs describe future jobs whose arrival times and durations are probabilistic, and whose utility to the submitting agents declines with completion time. The arrival and duration distributions, as well as the utility functions, are considered private customer information and are reported by strategic agents to a scheduler that is optimizing for social welfare. We design pricing, scheduling, and eviction mechanisms that incentivize truthful reporting of SoWs. An important challenge is maintaining incentives despite the possibility of the platform becoming saturated. We introduce a framework to reduce scheduling under uncertainty to a relaxed scheduling problem without uncertainty. Using this framework, we tackle both adversarial and stochastic submissions of statements of work, and obtain logarithmic and constant competitive mechanisms, respectively.

==> abstract-new.tex <==
Cloud computing customers often submit repeating jobs and computation pipelines on \emph{approximately} regular schedules, with arrival and running times that exhibit variance. % MB: maybe replace ''low variance'' with ''that varies in length" or something like that - but then we might need to also change the later stuff
%This is especially true for training machine learning models, where compute requirements are determined by the availability and quantity of training data at execution time.
%
This pattern, typical of training tasks in machine learning, allows prediction of future job requirements -- but only partially.
%
%Focusing on this pattern,
%which allows for some advance predictability by the submitting customers,
We develop a model of cloud computing platforms that receive statements of work that describe future jobs whose arrival times and durations are probabilistic. 
%and whose utility 
%to the submitting agents 
%declines with completion time. 
The arrival and duration distributions, as well as the mapping from completion time to customer value, are private information reported by % the submitting
strategic agents to an online scheduler optimizing for welfare.

We design pricing, scheduling, and eviction mechanisms that incentivize truthful reporting of statements of work.
%
%An important technical challenge is to maintain
%
%% BL: I changed `truthfulness' to `our incentive properties' in the next sentence, since technically our mechanism is not truthful (only approximately truthful).  The sentence above seems okay.
%
%\bledit{Our incentive properties are maintained even when the platform %is overbooked
%becomes saturated due to
%%many jobs simultaneously requiring more resources than predicted.
%%unlikely %low probability
%%events where
%larger-than-anticipated
%realized demand.}
%
%
An important challenge is maintaining incentives despite the possibility of the platform becoming saturated.
%
We introduce a framework
%Our solution takes the form of a
%general framework that
to reduce
%reduction from
scheduling under uncertainty to a relaxed scheduling problem without uncertainty.
%
Using this framework,
we tackle both adversarial and stochastic submissions of statements of work,
and obtain logarithmic and constant competitive mechanisms, respectively.
%
%total realized demand being larger than anticipated.}
%joint job realizations.
%
%
%to
%%the problem
%%the mechanism design task
%%to finding
%a posted-price scheduler in a relaxed scheduling environment with no uncertainty.
%in job requirements.
%\mbc{maybe replace by: “We first present a general framework that reduces our problem with uncertainty in job requirements, to the problem of designing a posted-price scheduler for a relaxed scheduling problem with no uncertainty.”}
%
%Using an algorithmic framework based on TODO,
%
%. In the adversarial case, {the competitive ratio of our mechanism
%social welfare achieved by our mechanism
%is logarithmic in the maximum %\blcomment{should we add: in the maximum job value and length \mbc{ratios}}.
%job utility and length.}
%When statements of work arrive stochastically from known distributions, our mechanism is $O(1)$-competitive.
%

